The Factuality of Large Language Models in the Legal Domain

This paper investigates the factuality of large language models (LLMs) as knowledge bases in the legal domain, in a realistic usage scenario: we allow for acceptable variations in the answer, and let the model abstain from answering when uncertain. First, we design a dataset of diverse factual questions about case law and legislation. We then use the dataset to evaluate several LLMs under different evaluation methods, including exact, alias, and fuzzy matching. Our results show that the performance improves significantly under the alias and fuzzy matching methods. Further, we explore the impact of abstaining and in-context examples, finding that both strategies enhance precision. Finally, we demonstrate that additional pre-training on legal documents, as seen with SaulLM, further improves factual precision from 63% to 81%.

==> sections/introduction_draft.tex <==
Language models (LMs) store knowledge from pre-training documents, allowing them to be queried with natural language (NL) rather than a formal language, unlike structured knowledge bases (KBs) \cite{petroni_language_2019, chang_language_2024}. This natural language interface democratizes access to knowledge for a larger number of users, particularly valuable in domain-specific areas where users may not master querying structured KBs \cite{hendrix_developing_1978}. In the legal domain, this includes both law experts, such as scholars, judges, lawyers, and paralegals, and laymen seeking information about legal problems\cite{boniol2020performance}. LMs can acquire and store more facts than KBs, as most of knowledge is stored in NL documents. This reduces the cost associated with manually populating KBs, as LMs can automatically store knowledge from pre-training documents without needing human supervision \cite{alkhamissi_review_2022}. While Wikidata is the largest structured KB available, it lacks comprehensive domain-specific knowledge \cite{weikum_machine_2020, zhang2022enriching}. Instead, Wikipedia articles, which LMs can store through pretraining, offer this knowledge.

The concept of language models as knowledge bases (LM-as-KB) was first introduced by \cite{petroni_language_2019}, showing that using BERT to retrieve facts in a cloze-style manner on the LAMA dataset outperforms traditional knowledge bases. Subsequent research \cite{heinzerling_language_2021} has shown that large language models (LLMs) with more than 10B parameters has the potential to store the entirety of Wikidata and retrieve facts using NL queries, although the accuracy of these queries can be sensitive to minor variations in query phrasing such as punctuation. Additionally, fine-tuning LMs or presenting them with query variants improves their robustness in retrieving facts \cite{jiang_how_2020, heinzerling_language_2021, adolphs_how_2021}.
LAMA \cite{petroni_language_2019} was the first dataset to benchmark LM-as-KB. However, to simplify the evaluation, it is limited to one token facts. Subsequent benchmarks have been developed to include more complex queries encompassing various types of knowledge \cite{bisk_piqa_2019, peng_copen_2022, lin_birds_2020, misra_comps_2023, elazar_measuring_2021}. Among these, KAMEL \cite{kalo_kamel_2022} proved to be more difficult than LAMA because the dataset contains multi-token facts, facts with literal values, broader range of knowledge and higher cardinality relations.

Early research on LM-as-KB primarily evaluated smaller models like BERT. However, the advent of large language models (LLMs) such as OpenAI's GPT models, Google's PALM models, and Meta's Llama models \cite{achiam2023gpt, chowdhery2022palm, touvron2023llama}, has revolutionized the field. These models exhibit emergent abilities useful for LM-as-KB, including few-shot prompting \cite{brown2020language} and calibration \cite{wei2022emergent}. LLMs can learn new tasks through few-shot prompting without requiring fine-tuning. Given that the performance of LM-as-KB improves significantly with prompt fine-tuning \cite{qin_learning_2021}, incorporating examples of queries in the prompt can enhance the factuality of LMs. Additionally, well-calibrated models can predict the correctness of their own responses, enabling self-evaluation of answers to factual queries \cite{kadavath_language_2022, geng_survey_2024}.

Despite their capabilities, LLMs are prone to \emph{hallucination} \cite{ji_survey_2023, suchanek2023knowledge}, producing factually incorrect answers in a disturbingly self-confident tone. While many studies have examined the factual accuracy of LLMs \cite{achiam2023gpt, wei_long-form_2024, muhlgay_generating_2024, hu_towards_2024, si_prompting_2023, min_factscore_2023, manakul_selfcheckgpt_2023, mallen_when_2023-1}, most have been generalist and not focused on domain-specific knowledge. Domain-specific knowledge poses unique challenges, such as: specific named entities that are unique to the domain (e.g. lawyer, judge), and that do not appear in abundance on the Internet (and hence in training data); relations that may not even be known to the general public (e.g. the judge who issues the majority opinion of case); facts that are specific to the domain (e.g. legal rules); and finally ways of phrasing that are typical for the jargon, but unusual on the Web as a whole (e.g. concurring or dissenting opinion). At the same time, domain-specific applications harbor a huge potential, as they can help users in areas that one-size-fits-all products do not reach.

In this paper, we focus on factual answers in the legal domain, motivated by both the risks and opportunities of using LLMs in this field \cite{bommasani_opportunities_nodate}. While existing benchmarks like LawBench \cite{fei_lawbench_2023} and LegalBench \cite{guha_legalbench_2023} evaluate LLMs on various legal tasks, LawBench is specific to Chinese law, and LegalBench does not include a legal knowledge task, limiting their applicability for probing LLMs on legal facts. The legal domain is particularly sensitive to hallucinations, as incorrect information can lead to harmful decisions \cite{dahl_large_2024}. Previous work often used strict evaluation criteria, accepting answers only if identical to the ground truth, which does not account for valid variations in response phrasing (“Bill Gates” is as valid an answer as "William Henry Gates III"). Additionally, earlier studies typically forced LLMs to provide answers, increasing the likelihood of hallucinations. In contrast, our approach allows models to abstain from answering when unsure, reducing the incidence of hallucination.

In our work, we systematically study and illuminate the factual accuracy of current LLMs in the legal domain. More precisely, we analyse
\begin{enumerate}
    \item Are all LLM equal towards the shortcomings (blindspots) of exact matching-based evaluation? Or they are certain LLM that are more penalized than others because of those shortcomings?
    \item Can the model abstain from generating incorrect answers?
    \item Do in-context examples increase the factuality of LLM? 
    \item Does extending an LLM to legal document improve the factuality of LLM?
\end{enumerate}


==> sections/related_work_notes.tex <==
\newpage

\appendix

Language models store both commonsense and factual knowledge contained in the pre-training corpus in their weights \cite{petroni_language_2019, chang_language_2024}. Therefore they can be queried as a knowledge base. However language models still lack several properties that KBs have, and this lack limits their usage as KBs.

\subsection{Scope}
Methods that query LM without fine-tuning the target answers nor injecting knowledge by updating the model parameters. Because they don't generalize well.
I am unsure about keeping methods using prompt-tuning. It seems that even when fine-tuning the prompts the gain in accuracy is much more important for objects seen during the fine-tuning than the ones only seen at test time \cite{qin_learning_2021} .

\subsection{Why LMs are considered as KB}
Because they showcased the following features \cite{petroni_language_2019, heinzerling_language_2021, chang_language_2024}:
\begin{itemize}
    \item Storage of a large number of entities, at least 100M \cite{heinzerling_language_2021}
    \item Soft of querying of facts
\end{itemize}

\subsection{Requirements of LMs to act like a KB}
First, LMs don't need to behave exactly like KBs. They need to ensure the critical features according to the use cases, especially those not covered by symbolic KBs.
\subsubsection{Complex queries}
\begin{itemize}
    \item 1-to-n relations
    \item Multihop inference
    \item Queries involving numerical ranges
    \item Facts qualified by time and location
\end{itemize}

\subsection{Notes on: Language Models as Knowledge Bases?}
BERT significantly outperformed KBs constructed from text on the task of object prediction \cite{petroni_language_2019}. This paper showed the potential of LM to capture knowledge from large-size corpora and to be an alternative to KBs extracted from text. Other findings of \cite{petroni_language_2019}:
\begin{itemize}
    \item The performance of BERT is high for 1-to-1 relations and low for N-to-M relations.
    \item Performance is correlated to the models' confidence about the first-ranked prediction. The prediction is often correct when BERT is highly confident about it.
    \item Sensitivity of the results to the query template
    \item Similar performance on factual and commonsense knowledge
    \item Templates are manually designed for each relation
\end{itemize}

\subsection{Aspects of knowledge stored by LMs}
\subsubsection{Domains}
The knowledge stored in LM covers a broad range of domains \cite{petroni_language_2019,chang_language_2024}: medical \cite{sung_can_2021}, movies \cite{penha2020does}

\subsubsection{Commonsense Knowledge}
It was shown \cite{davison_commonsense_2019} that LMs can mine commonsense knowledge without any further fine-tuning.
Out-of-scope because it is difficult to disambiguate commonsense knowledge.

\subsubsection{Triples}
So far the only form of knowledge probed from LMs is triples (s,p,o).

\subsubsection{Knowledge size}
KBs store a very large size of knowledge. For example, Wikidata has 109,366,313 entity (18/04/24). Can an LM store the same amount of knowledge and how? \cite{heinzerling_language_2021} suggests an approach to store millions of entities.
According to \cite{heinzerling_language_2021} LLMs of size larger than 10B are capable of storing most of a KB of the size of Wikidata and even all of it.

\subsection{How to query LMs?}
The accuracy of the query result depends on the prompt. Several methods have been developed to search for prompts to increase the accuracy. 
Manual prompts are proven to be suboptimal \cite{jiang_how_2020}. The paper also shows that syntactically simpler prompts and prompts with words frequent in the pertaining corpus tend to perform the best. Also there is no single prompt that is the best for retrieving all objects because ensembling prompts always give better results. Performance gain can be up to 23\% by updating one simple word in the prompt. For example x plays in→at y position.
Another simple trick to extract more facts is to query by example. \cite{adolphs_how_2021} introduces a an example sentence, of the sentence to query, right before the manual prompt. This approach outperforms the ensemble of prompts \cite{jiang_how_2020} on LAMA \cite{petroni_language_2019}. 
\cite{heinzerling_language_2021} proofs that LMs are very sensitive to small query changes such as punctuation. Robustness is increased by fine-tuning the LM on hundreds of examples from the query variants, because fine-tuning increases the embeddings similarity between the orginial query and its variant. So we can expect that a LM good at paraphrasing would be robust to query variants, and therefore the same fact can be queried using different sentences. 
\subsubsection{Mixture of soft prompts}
In \cite{qin_learning_2021} they fine-tune an LM on pairs $(x,y)$ of a relation and evaluated on the held-out pairs of the same relation. The prediction target is the object $y$. The prompt can be a natural language prompt as in \cite{petroni_language_2019} or a soft prompt where the tokens are vectors in the same space as tokens embeddings $\mathbb{R}^d$. The number of tokens is fixed and their vectors are tuned.
An equivalent alternative is to start from a hard prompt and perturb the embeddings of each token by a small vector. The perturbation vectors are tuned.
Similarly to \cite{jiang_how_2020} they use an ensemble of prompts. The soft prompts are ensembled by a mixture-of-experts instead of product-of-experts \cite{jiang_how_2020}. 
Earlier works used encoder-only LMs, while this work experiment also with encoder-decoder LMs in particular BART. The encoder-decoder poses the challenge of generating multi-tokens answers while the ground truth has only one token. So they constrain the decoder to stop after generating one token.
Tuning the prompts outperforms informed prompts even when initializing with random vectors \cite{qin_learning_2021}. 


\subsection{Consistency}
In \cite{elazar_measuring_2021} LMs has low factual consistency.

\subsection{Output space}

\subsection{Explanation of the good performance}
Potential reasons to explain the good performance of LM as KB:
\begin{itemize}
    \item The LM learned associations between subjects, relations, and objects from the frequency of their co-occurrences in the pre-training dataset.
    \item Biased prompts \cite{cao_knowledgeable_2021}
\end{itemize}

\subsection{Self-evaluation}
Larger models can assess the correctness of their answers to factual queries \cite{kadavath_language_2022}. The assessment is possible if the models are well calibrated so the probability of the output can assess the correctness of the output. Moreover they also \cite{kadavath_language_2022} can estimate the probability of "I know" the answer before generating the answer in certain settings.

\subsection{Calibration}
\cite{kadavath_language_2022} shows cases where LMs outputs are well calibrated: diverse multiple choice and true/false questions. 

\subsection{Challenging queries}
\cite{kalo_kamel_2022}  (2022) builds a more challenging benchmark for LM-as-KB. The performance drops from 52.90\% on LAMA to 17.62\% on KAMEL. The factors of difficulty are: multi-token answers, facts with literal values, broader range of knowledge and higher cardinality relations.
\subsubsection{Multiple objects relations}
Many papers make a certain design choice to deal with multiple objects relations:
\begin{itemize}
    \item \cite{petroni_language_2019} deals with it at evaluation time
    \item \cite{heinzerling_language_2021} create a synthetic datasets where only one object is kept for a pair of subject, predicates. It is not mentioned how the remained object is selected.
\end{itemize}

\subsubsection{Multi-token answers}
\begin{itemize}
    \item Challenging for \cite{petroni_language_2019}, where they limited the experiments to single-token answers.
    \item One of the reasons \cite{petroni_language_2019} limits the prediction to object slot and doesn't consider relation slot
    \item  \cite{heinzerling_language_2021} generates multiple tokens responses and evaluate via exact matching. The generation is done by beam-search of size 10.
\end{itemize}

\subsubsection{Literal values}
\begin{itemize}
    \item years
\end{itemize}

\subsubsection{Numerical commonsense}
\begin{itemize}
    \item LMs (as of 2020) strugles on numerical commonsense knowledge \cite{lin_birds_2020}. For example it predicts that a bird has fours legs instead of two legs. Even with fine-tuning the performance is still significantly lower than human performance.

\subsubsection{Conceptual knowledge}
It might not be explicitly mentioned in the pre-training corpus. This difference w.r.t factual knowledge might require a different mechanism from LMs to store and probe conceptual knowledge. The COPEN \cite{peng_copen_2022} proves that conceptual knowledge is challenging from LMs (as of 11/2022) and in \cite{misra_comps_2023} (as of 02/23).
Examples from COPEN:
\begin{itemize}
    \item Inter Milan is conceptually similar with [Milan, Milan Fashion Week, \textbf{Pohang Steelers}, Series A]
    \item Choose the concept that best fits the context for Dolly according to the context: Dolly is running on the grassland. Dolly is a(n) [\textbf{animal}, mammal, horse]
\end{itemize}




\end{itemize}

\subsubsection{Affordance}
Quote
\begin{quote}
    We found that only one NLM (GPT-3) was sensitive to the affordedness of actions. Moreover, GPT-3 accounted for only one third of the effect of affordedness on human sensibility judgments. These results imply that people use processes that go beyond distributional statistics to understand linguistic expressions, and that NLP systems may need to be augmented with such capabilities.\cite{jones_distrubutional_2022}
\end{quote}
\subsubsection{Unseen entities}
The performance dropped on entities not present in the fine-tuning dataset \cite{qin_learning_2021}

\subsection{Understanding the failures of LM as KB}
\subsubsection{Content of the prompt}
In \cite{poerner_e-bert_2020} it relies on the surface form patterns or semantic similarity between the words in the prompt and the correct answer. The context in the prompt can mislead the LM to output the wrong answer \cite{pandia2021sorting, kassner_edin_2022}.  
\subsubsection{Frequency of facts in the pre-training corpus}
Small LMs memorize more accurately facts that are frequent in the pre-training corpus in comparison to rare facts \cite{kassner_are_2020, kandpal_large_2023}.   Scaling the LMs size only improves its factual accuracy on popular entities and still struggles with long tail entities  \cite{mallen_when_2023}
\subsubsection{Generalization vs. Memorization}
LMs are not as good at generalizing (inference) facts as they are at memorizing facts seeing in the pre-training corpus \cite{kassner_are_2020}. However they can generalize better on facts observed in context (prompt) after pre-training \cite{misra_comps_2023}.
\subsubsection{Reasoning vs. Association}
LM has issues with
\begin{itemize}
    \item Negation \cite{kassner_are_2020}
    \item Mispriming
    \item Pattern heuristics 
\end{itemize}

\subsection{Techniques to improve LM-as-KB}
\subsubsection{Retrieval-augmented LM}
\cite{mallen_when_2023} outperforms larger LMs on long-tail entities.


\subsection{LM Capacity for storing facts}
Accuracy on factual queries increases with the model size \cite{heinzerling_language_2021}. On the other hand it drops when the the number of facts to memoriz increases. 
The capacity of the LM depends also on two factors: number of entities and the entropy of their distribution \cite{heinzerling_language_2021}.  The paper shows that the surface form representation of entities is the most robust w.r.t entities number. 

\subsection{LMs vs. KBs}
\subsubsection{Pros of LMs over KBs}
\begin{itemize}
    \item Natural language interface to structured data \cite{hendrix_developing_1978}: Flexibility when querying. LMs can be queried with NL while KBs need to be queried using a formal language.
    \item Self-reflection (I am not sure if KBs have this property)
\end{itemize}

\subsubsection{Pros of KBs over LMs}
\begin{itemize}
    \item Guarantees for the success and correctness of a query, because both the query and its output are unambiguous
    \item KBs are less subject to reporting bias than LMs
\end{itemize}

\subsection{Benchmarks}
\subsubsection{LegalBench}
LegalBench is the largest benchmark dataset for legal NLP, however, it lacks knowledge tasks.
\subsubsection{LawBench}
Chinese benchmark
\subsubsection{HELM}
Holistic Evaluation of Language Models. It has tasks that span multiple domains such as law.
\subsubsection{TruthfulQA}
TruthfulQA: Measuring How Models Mimic Human Falsehoods. It contains questions in the legal domain. The ground truth answers are sentences instead of entities like most of the other benchmarks.

\subsubsection{KAMEL}
Introduced in \cite{kalo_kamel_nodate} as a more challenging alternative for LAMA. KAMEL is also based on Wikidata and Wikipedia. More domains and multi-token entities.
\subsubsection{PIQA}
For physical commonsense \cite{bisk_piqa_2019}
\subsubsection{COPEN}
A benchmark for conceptual knowledge \cite{peng_copen_2022}.
\subsubsection{NumerSense}
Numerical reasoning \cite{lin_birds_2020}.
\subsubsection{COMPS}
Conceptual knowledge \cite{misra_comps_2023}. It deals with property inheritance
\subsubsection{CONCEPTNET}
\subsubsection{CSQA}
\subsubsection{PARAREL}
For factual consistency \cite{elazar_measuring_2021}
\subsubsection{KILT}
\cite{petroni_kilt_2021} contains multiple knowledge tasks. The tasks that are relevant to the basic formulation of LM-as-KB are:
\begin{itemize}
    \item Slot Filling (SF)
    \item Zero Shot RE from \cite{levy_zero-shot_2017}
    \item T-Rex \cite{elsahar_t-rex_2018}
    \item HotpotQA (not sure if all answers are entities)
    \item Natural Questions: I can keep answers that match exactly the title of Wikipedia page
\end{itemize}
\subsubsection{WebQuestions}
Natural language questions that can be answered from Freebase \cite{berant2013semantic}
\subsubsection{ComplexWebQuestion}
Same as above but more complex \cite{talmor2018web}
\subsubsection{GraphQ}
\cite{su2016generating} "array of question characteristics are formalized, including structure complexity, function, commonness, answer cardinality, and paraphrasing".
\subsubsection{KQApro}
"Dataset for Complex KBQA including ~120K diverse natural language questions." \cite{cao2020kqa}
\subsubsection{GRAILQA}
"a large-scale, high-quality KBQA dataset containing 64K questions with diverse characteristics
to support the development and evaluation of KBQA models with stronger generalization at all three levels" \cite{gu2021beyond} 
\subsubsection{MKQA}
\cite{longpre2021mkqa} 
"We introduce Multilingual Knowledge Questions and Answers (MKQA), an open-domain question answering evaluation set comprising 10k question-answer pairs aligned across 26 typologically diverse languages (260k question-answer pairs in total)". Answers are entities from Wikidata.


\subsection{Evaluation}
\begin{itemize}
    \item Exact matching
    \item Tokens F1 score
    \item P@k
    \item Hits@k
    \item MRR
    \item Conceptual consistency \cite{sahu_unpacking_2022}

\end{itemize}


\subsection{Constrained decoding}
The generation methodology in \cite{elazar_measuring_2021} uses constrained decoding. Since the evaluation is limited to single-token objects, constrained decoding is implemented by limiting the target vocabulary to only tokens of valid objects. 


\begin{itemize}
    \item \href{https://scholar.google.com/scholar_url?url=https://arxiv.org/abs/2307.06908&hl=en&sa=T&oi=gsb&ct=res&cd=0&d=5608570652501844927&ei=BaciZpOKC5jJy9YP2cuf6AE&scisig=AFWwaeYEkZ6qITh2uqg7v_14zMxg}{Generating benchmarks for factuality evaluation of language models}
    \item \href{https://aclanthology.org/2023.emnlp-main.416.pdf}{Lazy-k Decoding: Constrained Decoding for Information Extraction}
    \item \href{https://aclanthology.org/2023.emnlp-main.674.pdf}{Grammar-Constrained Decoding for Structured NLP Tasks without Finetuning}
    \item \href{https://aclanthology.org/2023.emnlp-main.905.pdf}{Self-Ensemble of N-best Generation Hypotheses by Lexically Constrained Decoding}
\end{itemize}

\subsection{LLM-based evaluation}
\cite{wang_evaluating_2023} shows that Exact Matching (EM) evaluation underestimates the model performance on QA compared to human evaluation.




\subsection{(Open) Research questions}
\subsubsection{On the quantity of knowledge stored by LMs}
\textbf{Idea:} We can accurately quantify the amount of knowledge (that can be expressed as triples) if we can query the LM to generate all the triples seen in the pertaining corpus. Check \cite{heinzerling_language_2021}

\section{Hallucination}
- Extrinsic hallucination
- A lack of consensus on hallucination definition and measuring framework \cite{venkit2024confidently}
- Poor correlation of metrics based on token overlap with human evaluation
\cite{ji_survey_2023}

==> tables/abstain_rate.tex <==
\begin{table}
\begin{tabular}{llrr}
\toprule
 & & \multicolumn{2}{c}{Abstain prompt} \\
Model & Prompt Strategy &  Without& With \\
\midrule
\multirow[t]{2}{*}{Saul} & Few-shot & 0.08 & 85.56 \\
 & Zero-shot & 0.00 & 39.81 \\
\cline{1-4}
\multirow[t]{2}{*}{Llama-2-7B} & Zero-shot & 0.99 & 83.22 \\
 & Few-shot & 0.07 & 4.45 \\
\cline{1-4}
\multirow[t]{2}{*}{Phi-3-mini-4k} & Zero-shot & 0.61 & 33.51 \\
 & Few-shot & 0.07 & 2.10 \\
\cline{1-4}
\multirow[t]{2}{*}{Gemma-7B} & Zero-shot & 8.89 & 30.46 \\
 & Few-shot & 0.43 & 11.78 \\
\cline{1-4}
\multirow[t]{2}{*}{Gemma-2B} & Zero-shot & 5.42 & 21.16 \\
 & Few-shot & 0.19 & 4.05 \\
\cline{1-4}
\multirow[t]{2}{*}{Mistral-7B} & Few-shot & 1.45 & 14.89 \\
 & Zero-shot & 0.82 & 5.77 \\
\cline{1-4}
\multirow[t]{2}{*}{RecurrentGemma-2B} & Zero-shot & 4.96 & 12.56 \\
 & Few-shot & 0.46 & 2.10 \\
\cline{1-4}
\multirow[t]{2}{*}{Llama-3-8B} & Few-shot & 0.08 & 4.82 \\
 & Zero-shot & 0.38 & 2.78 \\
\cline{1-4}
\bottomrule
\end{tabular}
\caption{Comparison between abstain rate under different prompting strategies, and with or without the abstain instruction: "If you don't know the answer, respond with "I don't know". \fms{May I suggest to report in Columns 3 and 4 both (1) abstention rate and (2) precision? No need for Figure 3 then...}}
\label{tab:abstain_rate}
\end{table}

